On Sampling Top-K Recommendation Evaluation

Recently, Rendle has warned that the use of sampling-based top-$k$ metrics might not suffice. This throws a number of recent studies on deep learning-based recommendation algorithms, and classic non-deep-learning algorithms using such a metric, into jeopardy. In this work, we thoroughly investigate the relationship between the sampling and global top-$K$ Hit-Ratio (HR, or Recall), originally proposed by Koren[2] and extensively used by others. By formulating the problem of aligning sampling top-$k$ ($SHR@k$) and global top-$K$ ($HR@K$) Hit-Ratios through a mapping function $f$, so that $SHR@k\approx HR@f(k)$, we demonstrate both theoretically and experimentally that the sampling top-$k$ Hit-Ratio provides an accurate approximation of its global (exact) counterpart, and can consistently predict the correct winners (the same as indicate by their corresponding global Hit-Ratios).

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> text/eval.tex <==
%\vspace*{-1.0ex}
\section{Experimental Results}
\label{experiments}

In this section, we experimentally study the sampling hit ratio $SHR@k$ and its corresponding global hit ratio $HR@K$ through different mapping functions $f$. Specifically, we aim to answer: 

%the following questions:

\begin{itemize}
    \item (Question 1) How does the dataset-independent mapping function $f$ help align $SHR@k$ with respect to $HR@f(k)$? 
    \item (Question 2) How do different factors, such as the top-$k$ location, varying the effect of the sampling scheme, and the sampling size affect the results?
    \item (Question 3) How does the algorithm-specific mapping function $f$  compare with other mapping functions? 
    \item (Question 4) How can the random sampling hit ratios be used to identify the winners of recommendation algorithms with respect to the corresponding global hit ratio?
\end{itemize}

% $(which potentially provides the lower bound for a specific algorithm on a given dataset, based on Beta distribution)

\begin{figure*}[th]
\begin{subfigure}{0.48\textwidth}
    \includegraphics[width=\textwidth, scale = 0.8]{Figures/FIG/VAE-N.png}
    \caption{Hit Ratios from the Global Top-$K$}
    \label{figure:ml-1m:global}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
    \includegraphics[width=\textwidth, scale = 0.8]{Figures/FIG/VAE-S.png}
    \caption{Hit Ratios from the Sampling Top-$k$}
    \label{figure:ml-1m:sample}
\end{subfigure}
\caption{ml-1m, n = 100}
\label{figure:ml-1m:Performance}
%\vspace*{-3.0ex}
\end{figure*}

\noindent{\bf Experimental Setup:}
We use four of the most commonly used datasets for recommendation studies, together with the {\texttt book-X} dataset, with a relatively large number of total items, for evaluating the effect of sampling size. The characteristics of these datasets are in Table~\ref{tab:datasets}. 

For the different recommendation algorithms, we use some of the most well-known and the state-of-the-art algorithms, including three non-deep-learning options: itemKNN~\cite{DeshpandeK@itemKNN};
ALS~\cite{hu2008collaborative}; and EASE~\cite{Steck_2019}; 
and three deep learning options:   
NCF~\cite{he2017neural};
MultiVAE~\cite{liang2018variational}; 
and NGCF~\cite{Wang_2019}. 
For each recommendation algorithm on a particular dataset, we report the result of only one sample run, as we found they are very close to the average of multiple run results. The default sampling method is sampling with replacement, unless explicitly stated. Also, we collect both sampling hit ratio $SHR@k$ ($k$ from $1$ to $n$, the sampling size) and global hit ratio $HR@K$ ($K$ from $1$ to $N$, the number of total items). In the figures, we also use {\em population} for $HR@K$ (global) and {\em sample} for $SHR@k$ curves. 
For the different mapping functions, we consider the linear (Formula~\ref{eq:fk1}), the bound (Formula~\ref{eq:bound_mid}), $Beta@1$ ($f(k;a=1)$, Formula~\ref{eq:uni_fk}), $Beta@0.5$ ($f(k;a=0.5)$, Formula~\ref{eq:fk}), and $Beta@P$ for the algorithm-specific mapping (Formula~\ref{recursive}). 
Below, we will report our experimental findings for the aforementioned questions. 
Due to the space limitation, we only report representative results here, and additional experimental results are openly available \footnote{\url{ https://github.com/dli12/KDD20-On-sampling-Top-K-Recommendation-Evaluation}}. 

\begin{small}
\begin{table}
  \caption{Dataset Statistics}
  \label{tab:datasets}
  \begin{tabular}{lcccc}
    \toprule
    \textbf{Dataset}&
    \textbf{Interactions}&
    \textbf{Users}&
    \textbf{Items}&\textbf{Sparsity}\\
    \midrule
    ml-1m  &1,000,209 & 6,040 &3,706&95.53$\%$\\
    pinterest-20& 1,463,581 & 55,187&9,916&99.73$\%$\\
    citeulike&204,986 &5,551&16,980&99.78$\%$ \\
    yelp& 696,865&25,677 &25,815&99.89$\%$ \\
    book-X& 786,690&11,325 &139,331&99.95$\%$\\
    \bottomrule
  \end{tabular}
\end{table}
\end{small}
%---------------- dataset--
% ml-1m \footnote{ \url{https://github.com/hexiangnan/neural_collaborative_filtering/tree/master/Data}} ~\cite{he2017neural}

% pinterest-20\footnote{\url{https://github.com/hexiangnan/neural_collaborative_filtering/tree/master/Data}} ~\cite{he2017neural}

% yelp\footnote{\url{https://github.com/duxy-me/ConvNCF/tree/master/Data}} ~\cite{he2018outer}

% citeulike\footnote{\url{https://github.com/tebesu/CollaborativeMemoryNetwork/tree/master/data}}
% ~\cite{ebesu2018collaborative}

% book-X\footnote{\url{http://www2.informatik.uni-freiburg.de/~cziegler/BX/}} ~\cite{Ziegler05}

%-----model---------%



\noindent{\bf Aligning Sampling and Global Hit Ratio $SHR$ and $HR$:} In this experiment, we provide two dual views of the alignment between sampling and global hit ratio (curves). Here, we report only the {\texttt MultiVAE} result on dataset {\textt ml-1m} in Figures~\ref{figure:ml-1m:Performance}. We use four different dataset-independent mapping functions, the linear, bound, $beta@1$ and $beta@0.5$, for the curve alignment. Figure~\ref{figure:ml-1m:global} maps the sampling curve $SHR@k$ to the global top-$K$ view by mapping $SHR@k$ to location $f(k)$ in the population/global top $K$ view, and compares them with the global $HR@K$ (population curve). Figure~\ref{figure:ml-1m:sample} maps the global curve $HR@K$ to the sampling top-$k$ view by $HR@K$ to the location $k$ (where $K=f(k)$) in the sampling top $k$ view, and then compares them with the sample $SHR@k$ (sampling curve). We observe that both bound and $beta@0.5$ achieve the best results from both views. The same observation holds on other recommendation algorithms and datasets. 

\noindent{\bf Key Factor Analysis (Top $k$, Sampling Factors and Sampling Size):}
To take a close look at different mapping functions,  
 we listed the sampling hit ratio $SHR$ at $k=1,2,5,10,20,50$ for sampling size $n-1=99$  and their corresponding global hit ratio $HR$ at $f(k)$ locations based on mapping functions, bound, $beta@1$ and $beta@0.5$ in Table\ref{table:varyingk1}.
 We show similar results for sampling size $n-1=999$. 
 In addition, we also consider three different sampling schemes: sampling with replacement (binom); sampling  without replacement (hyper); and sampling without replacement using only irrelevant items (actual).
 We made the following observations. (1) The differences between the sampling and the global $|SHR@k-HR@f(k)$ are fairly small, with the bound and $Beta@0.5$ more accurate; (2) When $k$ becomes larger, the results are more accurate.  (3) The results on the sampling with replacement and without replacement are very close to each other. Sampling with only irrelevant items, and the Global, which ranks only the irrelevant items, both lead to higher hit ratios. But the mapping function works equally well for this situation. (4) When sampling size increases (from $n=100$ to $n=1000$), the error also reduces. We further confirm this using Figure~\ref{fig:book_X}, which varies $n$ from $50$ to $1000$ on {\texttt book-X} dataset with more $139K$ items. When $n$ increases, the sampling hit ratio curve converges to the global hit ratio (population) rather quickly. 
 
 \begin{figure}[th]
    \includegraphics[width=\linewidth, scale = 0.9]{Figures/explain/NCF_X.png}
\caption{book-X:NeuMF}
\label{fig:book_X}
\end{figure}

 \noindent{\bf Dataset-independent vs algorithm-specific mapping:} Table~\ref{tab:MappingCompare} compares different dataset-independent mapping functions with the algorithm-specific one, $Beta@P$.  We compare both overall average absolute error $(\sum_{k=1}^n |HR@f(k)-SHR@k|)/n)$, the overall average relative error $(\sum_{k=1}^n (|HR@f(k)-SHR@k|/SHR@k)/n$, the errors at the top $1$, i.e., $|HR@f(1)-SHR@1|$ and $|HR@f(1)-SHR@1|/SHR@1$, and the errors between the top $2$ and $10$.  
 We observe that the algorithm-specific mapping function $Beta@P$ achieves the most minimal errors, over all.  However, the dataset-independent measures, such $Beta@0.5$, obtain comparable results and perform better when $k$ is small. We believe one of the underlying reasons is that $Beta@P$ aims to fit all the users (including those on the lower rank), and the fitting of Beta distribution has limitations. Thus, we consider that the dataset-independent mapping functions, such as $Beta@0.5$, can be a relatively cost-effective way to align sampling and global top-$k$ hit ratio curves. 
 
 % i.e., $\sum_{k=2}^10|HR@f(k)-SHR@k|/9$ and $\sum_{k=2}^10(|HR@f(k)-SHR@k|/SHR@k)/9$.
 
\noindent{\bf Predicting Winners (and Relative Performance):}
In Table~\ref{tab:consist}, we demonstrate the effectiveness of using sampling hit ratio $SHR@k$ to predict the recommendation algorithm performance when using the global hit ratio $HR@f(k)$.  We compare the performance of the three most competitive recommendation methods on the four commonly used datasets. We also vary the $k$ from $1$ to $50$ for sampling size $n-1=99$. Throughout all these cases, $SHR@k$ and $HR@f(k)$ all {\em consistently} predict the same and correct winners. Specifically, if an algorithm has the highest $SHR@k$, then it has the highest $HR@f(k)$ as well.  In fact, their relative orders are also mostly consistent besides the winners. 

%  How the dataset-independent mapping function $f$ help align $SHR@k$ with respect to $HR@f(k)$? 
%     \item (Question 2) What is the effect of random sampling with or without replacement and what is effect of sampling only irrelevant items as being done in ~\cite{}?
%     \item (Question 3) How the dataset-dependent mapping function $f$ compare with other mapping functions?
%     \item (Question 4) How the random sampling hit ratios can be used to the winners of recommendation algorithms with respect to the corresponding global hit ratio?
%     \item (Question 5) How does the sampling size $n$ affect the alignment between global and sampling hit ratios?
    


% \begin{subfigure}{0.48\textwidth}
%     \includegraphics[width=0.85\textwidth, height =0.65\textwidth]{Figures/FIG/EASE-ML1M-N.png}
%     \caption{Sampling}
%     \label{figure:ml-1m:sample}
% \end{subfigure}
% \begin{subfigure}{0.48\textwidth}
%     \includegraphics[width=0.85\textwidth, height =0.65\textwidth]{Figures/FIG/EASE-ML1M-S.png}
%     \caption{Population}
%     \label{figure:ml-1m:population}
% \end{subfigure}
% \begin{subfigure}{0.48\textwidth}
%     \includegraphics[width=0.85\textwidth, height =0.65\textwidth]{Figures/FIG/KNN-YELP-N.png}
%     \caption{Sampling}
%     \label{figure:ml-1m:sample}
% \end{subfigure}
% \begin{subfigure}{0.48\textwidth}
%     \includegraphics[width=0.85\textwidth, height =0.65\textwidth]{Figures/FIG/KNN-YELP-S.png}
%     \caption{Population}
%     \label{figure:ml-1m:population}
% \end{subfigure}
% \begin{subfigure}{0.48\textwidth}
%     \includegraphics[width=0.85\textwidth, height =0.65\textwidth]{Figures/FIG/NCF-YELP-N.png}
%     \caption{Sampling}
%     \label{figure:ml-1m:sample}
% \end{subfigure}
% \begin{subfigure}{0.48\textwidth}
%     \includegraphics[width=0.85\textwidth, height =0.65\textwidth]{Figures/FIG/NCF-YELP-S.png}
%     \caption{Population}
%     \label{figure:ml-1m:population}
% \end{subfigure}
% \caption{ml-1m}
% \label{figure:ml-1m:Performace}
% \end{figure*}


% \section{Result}
%-------------ml-1m, n=100----------%
\begin{small}
\begin{table*}[th]
    \caption{Varying Sampling Top $k$  on MultiVAE:ml-1m:n=100}
    \label{table:varyingk1}
    \begin{minipage}{0.32\textwidth}
      \caption*{binom(with replacement)}
      \centering
    \begin{tabular}{|l|cccc|}
    \hline
    \textbf{k}&
    \textbf{SHR}&
    \textbf{bound}&
    \textbf{beta@1}&
    \textbf{beta@0.5}\\
    \hline
1&0.1031&0.0442&0.1116&0.0829\\
2&0.2041&0.1700&0.2185&0.2012\\
5&0.4157&0.4050&0.4334&0.4209\\
10&0.6200&0.6204&0.6323&0.6258\\
20&0.7992&0.8012&0.8050&0.8028\\
50&0.9651&0.9682&0.9684&0.9682\\
    \hline
  \end{tabular}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \caption*{hyper(without replacement)}
        \begin{tabular}{|l|cccc|}
    \hline
    \textbf{k}&
    \textbf{SHR}&
    \textbf{bound}&
    \textbf{beta@1}&
    \textbf{beta@0.5}\\
    \hline
1&  0.1012& 0.0442&	0.1116&	0.0829\\
2&	0.1964&	0.1700&	0.2185&	0.2012\\
5&	0.4119&	0.4050&	0.4334&	0.4209\\
10&	0.6157&	0.6204&	0.6323&	0.6258\\
20&	0.7975&	0.8012&	0.8050&	0.8028\\
50&	0.9661&	0.9682&	0.9684&	0.9682\\
    \hline
  \end{tabular}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \caption*{actual(training data rank bottom)}
        \begin{tabular}{|l|cccc|}
    \hline
    \textbf{k}&
    \textbf{SHR}&
    \textbf{bound}&
    \textbf{beta@1}&
    \textbf{beta@0.5}\\
    \hline
1&	0.2101&	0.1608&	0.2540&	0.2161\\
2&	0.3349&	0.3199&	0.3810&	0.3555\\
5&	0.5533&	0.5603&	0.5889&	0.5768\\
10&	0.7164&	0.7295&	0.7391&	0.7334\\
20&	0.8531&	0.8661&	0.8690&	0.8674\\
50&	0.9757&	0.9800&	0.9803&	0.9798\\
    \hline
  \end{tabular}
    \end{minipage}
\end{table*}
\end{small}
%---------ml-1m,n=1000------
\begin{small}
\begin{table*}[th]
    \caption{Varying Sampling Top $k$ on MultiVAE:ml-1m:n=1000}
        \label{table:varyingk2}
    \begin{minipage}{0.32\textwidth}
      \caption*{binom(with replacement)}
      \centering
    \begin{tabular}{|l|cccc|}
    \hline
    \textbf{k}&
    \textbf{SHR}&
    \textbf{bound}&
    \textbf{beta@1}&
    \textbf{beta@0.5}\\
    \hline
10&	0.1091&	0.0998&	0.1116&	0.1089\\
20&	0.2126&	0.2124&	0.2185&	0.2174\\
50&	0.4281&	0.4306&	0.4334&	0.4318\\
100&	0.6293&	0.6303&	0.6316&	0.6316\\
200&	0.8036&	0.8043&	0.8050&	0.8046\\
500&	0.9672&	0.9682&	0.9684&	0.9684\\
    \hline
  \end{tabular}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \caption*{hyper(without replacement)}
        \begin{tabular}{|l|cccc|}
    \hline
    \textbf{k}&
    \textbf{SHR}&
    \textbf{bound}&
    \textbf{beta@1}&
    \textbf{beta@0.5}\\
    \hline
10&	0.1096&	0.0998&	0.1116&	0.1089\\
20&	0.2126&	0.2124&	0.2185&	0.2174\\
50&	0.4290&	0.4306&	0.4334&	0.4318\\
100&	0.6315&	0.6303&	0.6316&	0.6316\\
200&	0.8060&	0.8043&	0.8050&	0.8046\\
500&	0.9677&	0.9682&	0.9684&	0.9684\\
    \hline
  \end{tabular}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \caption*{actual(training data rank bottom)}
        \begin{tabular}{|l|cccc|}
    \hline
    \textbf{k}&
    \textbf{SHR}&
    \textbf{bound}&
    \textbf{beta@1}&
    \textbf{beta@0.5}\\
    \hline
10&	0.2417&	0.2407&	0.2540&	0.2495\\
20&	0.3682&	0.3704&	0.3810&	0.3770\\
50&	0.5776&	0.5861&	0.5889&	0.5874\\
100&	0.7286&	0.7381&	0.7389&	0.7389\\
200&	0.8570&	0.8684&	0.8690&	0.8689\\
500&	0.9747&	0.9800&	0.9803&	0.9803\\
    \hline
  \end{tabular}
    \end{minipage}
\end{table*}
\end{small}

%----- YELP--------%
% \begin{small}
% \begin{table*}[th]
%     \caption{MultiVAE:yelp:n=100}
%     \begin{minipage}{0.32\textwidth}
%       \caption*{binom}
%       \centering
%     \begin{tabular}{|l|cccc|}
%     \hline
%     \textbf{k}&
%     \textbf{SHR}&
%     \textbf{bound}&
%     \textbf{beta@1}&
%     \textbf{beta@0.5}\\
%     \hline
% 1&	0.2574&	0.2006&	0.3111&	0.2691\\
% 2&	0.4050&	0.3879&	0.4450&	0.4194\\
% 5&	0.6242&	0.6308&	0.6518&	0.6417\\
% 10&	0.7748&	0.7789&	0.7853&	0.7820\\
% 20&	0.8913&	0.8933&	0.8952&	0.8941\\
% 50&	0.9746&	0.9755&	0.9755&	0.9755\\
%     \hline
%   \end{tabular}
%     \end{minipage}
%     \begin{minipage}{0.32\textwidth}
%       \centering
%         \caption*{hyper}
%         \begin{tabular}{|l|cccc|}
%     \hline
%     \textbf{k}&
%     \textbf{SHR}&
%     \textbf{bound}&
%     \textbf{beta@1}&
%     \textbf{beta@0.5}\\
%     \hline
% 1&	0.2586&	0.2006&	0.3111&	0.2691\\
% 2&	0.4031&	0.3879&	0.4450&	0.4194\\
% 5&	0.6241&	0.6308&	0.6518&	0.6417\\
% 10&	0.7759&	0.7789&	0.7853&	0.7820\\
% 20&	0.8915&	0.8933&	0.8952&	0.8941\\
% 50&	0.9749&	0.9755&	0.9755&	0.9755\\
%     \hline
%   \end{tabular}
%     \end{minipage}
%     \begin{minipage}{0.32\textwidth}
%       \centering
%         \caption*{actual}
%         \begin{tabular}{|l|cccc|}
%     \hline
%     \textbf{k}&
%     \textbf{SHR}&
%     \textbf{bound}&
%     \textbf{beta@1}&
%     \textbf{beta@0.5}\\
%     \hline
% 1&	0.2757&	0.2154&	0.3237&	0.2837\\
% 2&	0.4137&	0.3987&	0.4550&	0.4297\\
% 5&	0.6297&	0.6355&	0.6550&	0.6455\\
% 10&	0.7781&	0.7812&	0.7876&	0.7834\\
% 20&	0.8917&	0.8941&	0.8959&	0.8950\\
% 50&	0.9749&	0.9757&	0.9757&	0.9756\\
%     \hline
%   \end{tabular}
%     \end{minipage}
% \end{table*}
% \end{small}

% \begin{small}
% \begin{table*}[th]
%     \caption{MultiVAE:yelp:n=1000}
%     \begin{minipage}{0.32\textwidth}
%       \caption*{binom}
%       \centering
%     \begin{tabular}{|l|cccc|}
%     \hline
%     \textbf{k}&
%     \textbf{SHR}&
%     \textbf{bound}&
%     \textbf{beta@1}&
%     \textbf{beta@0.5}\\
%     \hline
% 10&	0.3049&	0.3005&	0.3111&	0.3070\\
% 20&	0.4433&	0.4407&	0.4450&	0.4434\\
% 50&	0.6488&	0.6494&	0.6518&	0.6507\\
% 100&	0.7854&	0.7846&	0.7853&	0.7850\\
% 200&	0.8952&	0.8950&	0.8952&	0.8951\\
% 500&	0.9754&	0.9755&	0.9755&	0.9755\\
%     \hline
%   \end{tabular}
%     \end{minipage}
%     \begin{minipage}{0.32\textwidth}
%       \centering
%         \caption*{hyper}
%         \begin{tabular}{|l|cccc|}
%     \hline
%     \textbf{k}&
%     \textbf{SHR}&
%     \textbf{bound}&
%     \textbf{beta@1}&
%     \textbf{beta@0.5}\\
%     \hline
% 10&	0.3033&	0.3005&	0.3111&	0.3070\\
% 20&	0.4413&	0.4407&	0.4450&	0.4434\\
% 50&	0.6495&	0.6494&	0.6518&	0.6507\\
% 100&	0.7851&	0.7846&	0.7853&	0.7850\\
% 200&	0.8949&	0.8950&	0.8952&	0.8951\\
% 500&	0.9756&	0.9755&	0.9755&	0.9755\\
%     \hline
%   \end{tabular}
%     \end{minipage}
%     \begin{minipage}{0.32\textwidth}
%       \centering
%         \caption*{actual}
%         \begin{tabular}{|l|cccc|}
%     \hline
%     \textbf{k}&
%     \textbf{SHR}&
%     \textbf{bound}&
%     \textbf{beta@1}&
%     \textbf{beta@0.5}\\
%     \hline
% 10&	0.3155&	0.3144&	0.3237&	0.3193\\
% 20&	0.4513&	0.4502&	0.4550&	0.4528\\
% 50&	0.6519&	0.6533&	0.6550&	0.6543\\
% 100&	0.7869&	0.7869&	0.7876&	0.7872\\
% 200&	0.8960&	0.8956&	0.8959&	0.8957\\
% 500&	0.9759&	0.9757&	0.9757&	0.9757\\
%     \hline
%   \end{tabular}
%     \end{minipage}
% \end{table*}
% \end{small}
% %------------------%
% \newpage


\begin{small}
\begin{table*}[th]
    \caption{Mapping Functions Comparison}
    \label{tab:MappingCompare}
    %\vspace*{-3.0ex}
    \begin{minipage}{0.48\textwidth}
      \caption*{MultiVAE:ml-1m}
      \centering
    \begin{tabular}{|l|cccccc|}
    \hline
    \textbf{Dataset}&
    \textbf{abs}&
    \textbf{rel}&
    \textbf{abs@1}&
    \textbf{rel@1}&
    \textbf{abs@2-10}&
    \textbf{rel@2-10}\\
    \hline
Linear&0.0058&0.0226&0.0992&0.9934&0.0391&0.1238\\
Bound&0.0024&0.0103&0.0596&0.5970&0.0100&0.0363\\
Beta@1&0.0034&0.0074&0.0118&0.1177&0.0165&0.0440\\
Beta@0.5&0.0019&0.0043&0.0169&0.1692&0.0052&0.0112\\
Beta@0.2&0.0018&0.0065&0.0356&0.3566&0.0060&0.0207 \\
Beta@P&0.0018&0.0052&0.0250&0.2504&0.0052&0.0146 \\
    \hline
  \end{tabular}
    \end{minipage}\hfill
%     \begin{minipage}{0.48\textwidth}
%       \centering
%         \caption*{EASE:ml-1m}
%         \begin{tabular}{|l|cccccc|}
%     \hline
%     \textbf{Dataset}&
%     \textbf{abs}&
%     \textbf{rel}&
%     \textbf{abs@1}&
%     \textbf{rel@1}&
%     \textbf{abs@2-10}&
%     \textbf{rel@2-10}\\
%     \hline
% Linear&0.0056&0.0211&0.1101&0.9666&0.0374&0.1118\\
% Bound&0.0025&0.0084&0.0500&0.4390&0.0092&0.0294\\
% Beta@1&0.0037&0.0081&0.0205&0.1802&0.0152&0.0408\\
% Beta@0.5&0.0019&0.0031&0.0055&0.0480&0.0040&0.0085\\
% Beta@0.2&0.0018&0.0047&0.0237&0.2078&0.0047&0.0137\\ 
% Beta@P&0.0017&0.0034&0.0141&0.1235&0.0027&0.0059\\ 
%     \hline
%   \end{tabular}
%     \end{minipage} \hfill
%     \begin{minipage}{0.48\textwidth}
%       \caption*{itemKNN:yelp}
%   \begin{tabular}{|l|cccccc|}
%     \hline
%     \textbf{Dataset}&
%     \textbf{abs}&
%     \textbf{rel}&
%     \textbf{abs@1}&
%     \textbf{rel@1}&
%     \textbf{abs@2-10}&
%     \textbf{rel@2-10}\\
%     \hline
% Linear&0.0057&0.0145&0.3019&0.9874&0.0240&0.0443\\
% Bound&0.0019&0.0035&0.0529&0.1731&0.0053&0.0086\\
% Beta@1&0.0040&0.0069&0.0612&0.2003&0.0230&0.0384\\
% Beta@0.5&0.0024&0.0036&0.0183&0.0599&0.0131&0.0212\\
% Beta@0.2&0.0015&0.0022&0.0113&0.0369&0.0067&0.0101\\ 
% Beta@P&0.0017&0.0023&0.0023&0.0075&0.0086&0.0135\\ 
%     \hline
%   \end{tabular}
%     \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
      \centering
        \caption*{NeuMF:yelp}
  \begin{tabular}{|l|cccccc|}
    \hline
    \textbf{Dataset}&
    \textbf{abs}&
    \textbf{rel}&
    \textbf{abs@1}&
    \textbf{rel@1}&
    \textbf{abs@2-10}&
    \textbf{rel@2-10}\\
    \hline
Linear&0.0057&0.0164&0.2329&0.9886&0.0300&0.0632\\
Bound&0.0019&0.0046&0.0606&0.2571&0.0061&0.0125\\
Beta@1&0.0038&0.0070&0.0414&0.1756&0.0221&0.0413\\
Beta@0.5&0.0020&0.0030&0.0032&0.0134&0.0112&0.0197\\

Beta@0.2&0.0015&0.0027&0.0253&0.1075&0.0057&0.0097 \\
Beta@P&0.0015&0.0024&0.0145&0.0617&0.0067&0.0106\\
    \hline
  \end{tabular}
    \end{minipage} 
    %\vspace*{-3.0ex}
\end{table*}
\end{small}

% \newpage



% \newpage
% \begin{figure*}[th]\label{fig:VAE-1m}
% \begin{subfigure}{0.48\textwidth}
%     \includegraphics[width=\textwidth]{Figures/explain/N_ML1M.png}
%     \caption{Sampling}
%     \label{figure:ml-1m:sample}
% \end{subfigure}
% \begin{subfigure}{0.48\textwidth}
%     \includegraphics[width=\textwidth]{Figures/explain/N_YELP.png}
%     \caption{Population}
%     \label{figure:ml-1m:population}
% \end{subfigure}
% \caption{ml-1m}
% \label{figure:ml-1m:Performace}
% \end{figure*}

\begin{scriptsize}

\begin{table*}[th]
    \caption{Predicting Winners (and Relative Performance)}
    \label{tab:consist}
    %\vspace*{-2.0ex}
    \begin{minipage}{0.48\textwidth}
      \caption*{ml-1m}
      \centering
    \begin{tabular}{|l|ccc|ccc|ccc|}
    \hline
    &
    \multicolumn{3}{c|}{\textbf{NeuMF}}&
    \multicolumn{3}{c|}{\textbf{MultiVAE}}&
    \multicolumn{3}{c|}{\textbf{EASE}}\\
    \hline
    k&SHR&bound& $\mathcal{B}$@.5 &SHR&bound&$\mathcal{B}$@.5&SHR&bound&$\mathcal{B}$@.5\\
    \hline
1	&0.208&	0.150&	0.205&		0.211&	0.160&	0.216 &\textbf{0.223}&	\textbf{0.173}	&\textbf{0.232}	\\
2&	0.326&	0.311&	0.347	&	0.343	&0.319	&0.355 &\textbf{0.349}&	\textbf{0.334}&\textbf{	0.370}	\\
5&	0.548&	0.555&	0.566&		0.555&	0.560&	0.576&\textbf{ 0.564}&\textbf{	0.573}&	\textbf{0.587}	\\
10&	0.715&	0.726&	0.731&		0.717&	0.729&	0.733 &\textbf{0.720}	&\textbf{0.733	}&\textbf{0.737}\\
20&	0.850&	0.863&	0.864	&	\textbf{0.854}&	\textbf{0.866}&	\textbf{0.867}& 0.847&	0.859	&0.860	\\
50&	0.972&	0.979&	0.979	&	\textbf{0.972}&	\textbf{0.980}&\textbf{	0.979} &0.955&	0.961&	0.961	\\
    \hline
  \end{tabular}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
      \centering
        \caption*{yelp}
 \begin{tabular}{|l|ccc|ccc|ccc|}
    \hline
    &
    \multicolumn{3}{c|}{\textbf{NeuMF}}&
    \multicolumn{3}{c|}{\textbf{MultiVAE}}&
    \multicolumn{3}{c|}{\textbf{EASE}}\\
    \hline
    k&SHR&bound&$\mathcal{B}$@.5&SHR&bound&$\mathcal{B}$@.5&SHR&bound&$\mathcal{B}$@.5 \\
    \hline
1&	0.234&	0.184&	0.248	&	0.262&	0.215&	0.283 &\textbf{0.275}&\textbf{0.228}&\textbf{0.295}\\
2	&0.369	&0.360	&0.392	&	0.404&	0.398&	0.429 &\textbf{0.418}&	\textbf{0.410}&	\textbf{0.442}	\\
5	&0.593	&0.600	&0.611	&	0.626&	0.635&	0.645 &\textbf{0.632}&	\textbf{0.642}&	\textbf{0.653}	\\
10&	0.753&	0.760&	0.764	&	0.775&	0.781&	0.783 &\textbf{0.777}&\textbf{	0.784}&	\textbf{0.787}	\\
20&	0.881&	0.885&	0.886	&	\textbf{0.892}&	\textbf{0.894}&	\textbf{0.895} &0.886&	0.888&	0.889\\
50	&\textbf{0.975}&\textbf{	0.976}&\textbf{	0.976}	&	0.974&	0.975&	0.975 &0.957&	0.957	&0.957\\
    \hline
  \end{tabular}
    \end{minipage}\hfill 
% \end{table*}
% \end{scriptsize}


% \begin{scriptsize}

% \begin{table*}[th]
%     \caption{Consistency}
    \begin{minipage}{0.48\textwidth}
      \caption*{pinterest-20}
      \centering
    \begin{tabular}{|l|ccc|ccc|ccc|}
    \hline
    &
    \multicolumn{3}{c|}{\textbf{NeuMF}}&
    \multicolumn{3}{c|}{\textbf{MultiVAE}}&
    \multicolumn{3}{c|}{\textbf{EASE}}\\
    \hline
    k&SHR&bound& $\mathcal{B}$@.5 &SHR&bound&$\mathcal{B}$@.5&SHR&bound&$\mathcal{B}$@.5\\
   \hline
1&	0.273&	0.201&	0.278	&	\textbf{0.316}&	\textbf{0.241}	&\textbf{0.321} &0.289&	0.222&	0.298\\
2	&0.436&	0.409&	0.448	&\textbf{	0.479}&\textbf{0.456}&\textbf{0.495}& 0.452&	0.425&	0.465\\
5	&0.701&	0.708&	0.722&		\textbf{0.729}	&\textbf{0.735}	&\textbf{0.747}& 0.705&	0.712&	0.724\\
10&	0.874&	0.883&	0.886&		\textbf{0.887}	&\textbf{0.894}&	\textbf{0.897} &0.868&	0.877&	0.880\\
20&	0.965&	0.968&	0.968	&	\textbf{0.970}&	\textbf{0.973}	&\textbf{0.973}& 0.959&	0.963	&0.963\\
50	&0.993&	0.993&	0.993&		\textbf{0.994}&	\textbf{0.994}&	\textbf{0.994}& 0.989	&0.989&	0.989\\
    \hline
  \end{tabular}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
      \centering
        \caption*{citeulike}
 \begin{tabular}{|l|ccc|ccc|ccc|}
    \hline
    &
    \multicolumn{3}{c|}{\textbf{NeuMF}}&
    \multicolumn{3}{c|}{\textbf{MultiVAE}}&
    \multicolumn{3}{c|}{\textbf{EASE}}\\
    \hline
    k&SHR&bound&$\mathcal{B}$@.5&SHR&bound&$\mathcal{B}$@.5&SHR&bound&$\mathcal{B}$@.5 \\
        \hline
1&	0.399&	0.427	&0.505	&	\textbf{0.488}&	\textbf{0.554}	&\textbf{0.615}& 0.464&	0.511	&0.577	\\

2&	0.583&	0.606&	0.632	&	\textbf{0.675}&	\textbf{0.707}	&\textbf{0.727} &0.641&	0.674&	0.697\\

5	&0.767	&0.774&	0.783	&	\textbf{0.828}	&\textbf{0.839}&	\textbf{0.845} &0.802&	0.811&	0.815\\

10&	0.871&	0.878	&0.880&	\textbf{0.910}&	\textbf{0.914}&	\textbf{0.916} &0.880&	0.886&	0.887\\

20&	0.940&	0.944&	0.944	&	\textbf{0.961}&	\textbf{0.962}	&\textbf{0.963} &0.934&	0.936&	0.936\\
50&	0.987&	0.987&	0.987	&	\textbf{0.992}&	\textbf{0.991}&	\textbf{0.991}& 0.969&	0.968	&0.968\\
    \hline
  \end{tabular}
    \end{minipage} 
\end{table*}
\end{scriptsize}

%-------------------------



% \begin{small}
% \begin{table*}[th]
%     \caption{book-X}
%      \centering
%     \begin{tabular}{|l|ccc|ccc|ccc|}
%     \hline
%     &
%     \multicolumn{3}{c|}{\textbf{NeuMF}}&
%     \multicolumn{3}{c|}{\textbf{MultiVAE}}&
%     \multicolumn{3}{c|}{\textbf{ALS}}\\
%     \hline
%     n&abs&rel&max rel&abs&rel&max rel&abs&rel&max rel \\
%     \hline
% 50&0.0046&0.0069&0.0893&0.0049&0.0068&0.0799&0.0057&0.0084&0.0623\\
% 100&0.0028&0.0042&0.0719&0.0027&0.0040&0.0777&0.0029&0.0046&0.0649\\
% 200&0.0015&0.0026&0.0897&0.0017&0.0028&0.0964&0.0015&0.0026&0.0949\\
% 500&0.0009&0.0014&0.0287&0.0009&0.0015&0.0962&0.0010&0.0017&0.0822\\
% 1000&0.0005&0.0006&0.0270&0.0005&0.0007&0.0427&0.0007&0.0011&0.0288\\
%     \hline
%   \end{tabular}
% \end{table*}
% \end{small}


% \newpage
% \begin{figure*}[th]\label{fig:book-X}
% \begin{subfigure}{0.48\textwidth}
%     \includegraphics[width=\textwidth,height=0.66\textwidth]{Figures/explain/NCF_X.png}
%     \caption{NeuMF}
%     \label{fig:book-ncf}
% \end{subfigure}
% \begin{subfigure}{0.48\textwidth}
%     \includegraphics[width=\textwidth,height=0.66\textwidth]{Figures/explain/ALS_X.png}
%     \caption{ALS}
%     \label{fig:book-als}
% \end{subfigure}
% \caption{book-X}
% \end{figure*}



% \begin{small}
% \begin{table*}[th]
%     \caption{ml-1m}
%       \centering
%     \begin{tabular}{|l|ccc|ccc|ccc|ccc|}
%     \hline
%     &
%     \multicolumn{3}{c|}{\textbf{NeuMF}}&
%     \multicolumn{3}{c|}{\textbf{MultiVAE}}&
%     \multicolumn{3}{c|}{\textbf{EASE}}&
%     \multicolumn{3}{c|}{\textbf{ALS}}\\
%     \hline
%     k&SHR&bound&beta@0.5&SHR&bound&beta@0.5&SHR&bound&beta@0.5&SHR&bound&beta@0.5 \\
%     \hline
% 1	&0.2081&	0.1502&	0.2058&		0.2119&	0.1608&	0.2161 &\textbf{0.2233}&	\textbf{0.1737}	&\textbf{0.2326}	&	0.2136	&0.1606	&0.2242\\
% 2&	0.3268&	0.3119&	0.3470	&	0.3430	&0.3199	&0.3555 &\textbf{0.3497}&	\textbf{0.3348}&\textbf{	0.3700}	&	0.3329&	0.3205&	0.3508\\
% 5&	0.5485&	0.5555&	0.5669&		0.5558&	0.5603&	0.5768&\textbf{ 0.5646}&\textbf{	0.5732}&	\textbf{0.5873}	&	0.5339&	0.5452&	0.5566\\
% 10&	0.7156&	0.7263&	0.7313&		0.7177&	0.7295&	0.7334 &\textbf{0.7207}	&\textbf{0.7339	}&\textbf{0.7374}	&	0.6942	&0.7053&0.7093\\
% 20&	0.8508&	0.8639&	0.8646	&	\textbf{0.8545}&	\textbf{0.8661}&	\textbf{0.8674}& 0.8477&	0.8594	&0.8604	&	0.8225&	0.8364	&0.8374\\
% 50&	0.9722&	0.9790&	0.9790	&	\textbf{0.9725}&	\textbf{0.9800}&\textbf{	0.9798} &0.9555&	0.9618&	0.9616	&	0.9315	&0.9364&	0.9364\\



%     \hline
%   \end{tabular}
% \end{table*}
% \end{small}


% \begin{small}
% \begin{table*}[th]
%     \caption{yelp}
%       \centering
%     \begin{tabular}{|l|ccc|ccc|ccc|ccc|}
%     \hline
%     &
%     \multicolumn{3}{c|}{\textbf{NeuMF}}&
%     \multicolumn{3}{c|}{\textbf{MultiVAE}}&
%     \multicolumn{3}{c|}{\textbf{EASE}}&
%     \multicolumn{3}{c|}{\textbf{ALS}}\\
%     \hline
%     k&SHR&bound&beta@0.5&SHR&bound&beta@0.5&SHR&bound&beta@0.5&SHR&bound&beta@0.5 \\
%     \hline
% 1&	0.2346&	0.1846&	0.2488	&	0.2623&	0.2154&	0.2837 &\textbf{0.2751}&	\textbf{0.2284}&	\textbf{0.2953}	&	0.2467&	0.1990&	0.2597\\
% 2	&0.3697	&0.3600	&0.3921	&	0.4049&	0.3987&	0.4297 &\textbf{0.4181}&	\textbf{0.4105}&	\textbf{0.4423}	&	0.3782&	0.3698&	0.3968\\
% 5	&0.5934	&0.6009	&0.6114	&	0.6263&	0.6355&	0.6455 &\textbf{0.6328}&	\textbf{0.6426}&	\textbf{0.6538}	&	0.5734&	0.5826	&0.5917\\
% 10&	0.7537&	0.7606&	0.7640	&	0.7751&	0.7812&	0.7834 &\textbf{0.7770}&\textbf{	0.7842}&	\textbf{0.7878}	&	0.7025&	0.7049&	0.7081\\
% 20&	0.8814&	0.8854&	0.8862	&	\textbf{0.8922}&	\textbf{0.8941}&	\textbf{0.8950} &0.8867&	0.8889&	0.8894	&	0.7972&	0.7994&	0.7999\\
% 50	&\textbf{0.9756}&\textbf{	0.9762}&\textbf{	0.9762}	&	0.9745&	0.9757&	0.9756 &0.9574&	0.9578	&0.9577	&	0.8756	&0.8759	&0.8758\\
%     \hline
%   \end{tabular}
% \end{table*}
% \end{small}

% \begin{small}
% \begin{table*}[th]
%     \caption{pinterest-20}
%       \centering
%     \begin{tabular}{|l|ccc|ccc|ccc|ccc|}
%     \hline
%     &
%     \multicolumn{3}{c|}{\textbf{NeuMF}}&
%     \multicolumn{3}{c|}{\textbf{MultiVAE}}&
%     \multicolumn{3}{c|}{\textbf{EASE}}&
%     \multicolumn{3}{c|}{\textbf{ALS}}\\
%     \hline
%     k&SHR&bound&beta@0.5&SHR&bound&beta@0.5&SHR&bound&beta@0.5&SHR&bound&beta@0.5 \\
%     \hline
% 1&	0.2734&	0.2019&	0.2780	&	\textbf{0.3106}&	\textbf{0.2417}	&\textbf{0.3219} &0.2899&	0.2223&	0.2981	&	0.2623	&0.1972	&0.2651\\
% 2	&0.4360&	0.4095&	0.4489	&\textbf{	0.4792}&\textbf{0.4560}&\textbf{0.4950}& 0.4529&	0.4275&	0.4656	&	0.4158	&0.3903&	0.4269\\
% 5	&0.7010&	0.7080&	0.7221&		\textbf{0.7296}	&\textbf{0.7351}	&\textbf{0.7477}& 0.7057&	0.7120&	0.7248&		0.6659&	0.6706&	0.6833\\
% 10&	0.8741&	0.8832&	0.8866&		\textbf{0.8876}	&\textbf{0.8948}&	\textbf{0.8977} &0.8688&	0.8776&	0.8807&		0.8298&	0.8381&	0.8416\\
% 20&	0.9651&	0.9685&	0.9688	&	\textbf{0.9706}&	\textbf{0.9737}	&\textbf{0.9739}& 0.9596&	0.9633	&0.9637&		0.9233&	0.9269&	0.9272\\
% 50	&0.9935&	0.9934&	0.9934&		\textbf{0.9946}&	\textbf{0.9947}&	\textbf{0.9947}& 0.9891	&0.9894&	0.9893&		0.9582	&0.9584&	0.9583\\
%     \hline
%   \end{tabular}
% \end{table*}
% \end{small}

% \begin{small}
% \begin{table*}[th]
%     \caption{citeulike}
%       \centering
%     \begin{tabular}{|l|ccc|ccc|ccc|ccc|}
%     \hline
%     &
%     \multicolumn{3}{c|}{\textbf{NeuMF}}&
%     \multicolumn{3}{c|}{\textbf{MultiVAE}}&
%     \multicolumn{3}{c|}{\textbf{EASE}}&
%     \multicolumn{3}{c|}{\textbf{ALS}}\\
%     \hline
%     k&SHR&bound&beta@0.5&SHR&bound&beta@0.5&SHR&bound&beta@0.5&SHR&bound&beta@0.5 \\
%     \hline
% 1&	0.3994&	0.4277	&0.5059	&	\textbf{0.4886}&	\textbf{0.5545}	&\textbf{0.6157}& 0.4648&	0.5118	&0.5779	&	0.2801&	0.2508	&0.3122\\

% 2&	0.5837&	0.6069&	0.6325	&	\textbf{0.6756}&	\textbf{0.7074}	&\textbf{0.7271} &0.6411&	0.6745&	0.6970	&	0.4208&	0.4174&	0.4460\\

% 5	&0.7674	&0.7748&	0.7838	&	\textbf{0.8285}	&\textbf{0.8398}&	\textbf{0.8458} &0.8024&	0.8117&	0.8150	&	0.6193&	0.6269&	0.6374\\

% 10&	0.8717&	0.8780	&0.8800	&	\textbf{0.9108}&	\textbf{0.9142}&	\textbf{0.9161} &0.8804&	0.8860&	0.8876&		0.7620&	0.7678&	0.7696\\

% 20&	0.9407&	0.9442&	0.9447	&	\textbf{0.9613}&	\textbf{0.9629}	&\textbf{0.9631} &0.9342&	0.9360&	0.9362&		0.8694&	0.8707&	0.8714\\
% 50&	0.9870&	0.9876&	0.9876	&	\textbf{0.9924}&	\textbf{0.9919}&	\textbf{0.9919}& 0.9690&	0.9688	&0.9688	&	0.9600&	0.9584&	0.9580\\
%     \hline
%   \end{tabular}
% \end{table*}
% \end{small}
